Reparameterized Variational Rejection Sampling

Traditional approaches to variational inference rely on parametric families of variational distributions, with the choice of family playing a critical role in determining the accuracy of the resulting posterior approximation. Simple mean-field families often lead to poor approximations, while rich families of distributions like normalizing flows can be difficult to optimize and usually do not incorporate the known structure of the target distribution due to their black-box nature. To expand the space of flexible variational families, we revisit Variational Rejection Sampling (VRS) [Grover et al., 2018], which combines a parametric proposal distribution with rejection sampling to define a rich non-parametric family of distributions that explicitly utilizes the known target distribution. By introducing a low-variance reparameterized gradient estimator for the parameters of the proposal distribution, we make VRS an attractive inference strategy for models with continuous latent variables. We argue theoretically and demonstrate empirically that the resulting method--Reparameterized Variational Rejection Sampling (RVRS)--offers an attractive trade-off between computational cost and inference fidelity. In experiments we show that our method performs well in practice and that it is well-suited for black-box inference, especially for models with local latent variables.

==> semi_algo.tex <==
See Algorithm~\ref{alg:semiunbiased}-\ref{alg:semibiased}.

\begin{algorithm}[t]
	\caption{Unbiased Sampler for $r_{\bphi_{1}, \bth}(\bz_{1})\ldots r_{\bphi_{N}, \bth}(\bz_{N})$. {\bf Input}: subsample indices $\{i_1,\ldots,i_M\}$, number of particles $S$, acc.~prob.~$\{a_{\bphi_n, \bth}(\bz_n)\}$, and proposals $\{q_{\bphi_n}(\bz_n)\}$.
		%%{\bf Output}: $S$ sets of samples $\{\bz_{i_1}^{1:S},\ldots,\bz_{i_M}^{1:S}\}$.
	}
	\label{alg:semiunbiased}
	\begin{algorithmic}[1]
       \For{$k \gets 1$ to $M$} \Comment{Initialize the number of samples for each item}
       	\State $s_k \gets 0$
       \EndFor
		\While{$\min\{s_1,\ldots,s_M\} < S$}
		    \For{$k \gets 1$ to $M$} \Comment{Compute how many particles left to draw}
		    	\State $w_k \gets \max\{S - s_k, 0\}$ 
		    \EndFor
		    \State $W = \sum_{k=1}^M w_k$
		    \For{$k \gets 1$ to $M$}
		        $j \sim {\rm Categorical}(\frac{w_1}{W},\ldots,\frac{w_M}{W})$ \Comment{Draw a random index based on the weights }
			    \State $n \gets i_j$
			    \State $\bz_n \sim q_{\bphi_n}(\bz_n)$  \Comment{Perform reject sampling}
				\If {$u < a_{\bphi_n, \bth}(\bz_n)$ where $u \sim {\rm Uniform}(0,1)$}  
					\State $s_j \gets s_j + 1$
					\State $\bz_{i_j}^{s_j} \gets \bz_n$
				\EndIf
		    \EndFor
		\EndWhile
		\State return $\{\bz_{i_1}^{1:S},\ldots,\bz_{i_M}^{1:S}\}$
	\end{algorithmic}
\end{algorithm}

\begin{algorithm}[t]
	\caption{Biased Sampler for $r_{\bphi_{1}, \bth}(\bz_{1})\ldots r_{\bphi_{N}, \bth}(\bz_{N})$. {\bf Input}: subsample indices $\{i_1,\ldots,i_M\}$, number of particles $S$, number of candidates $S'$,  acc.~prob.~$\{a_{\bphi_n, \bth}(\bz_n)\}$, and proposals $\{q_{\bphi_n}(\bz_n)\}$.
		%%{\bf Output}: $S$ sets of samples $\{\bz_{i_1}^{1:S},\ldots,\bz_{i_M}^{1:S}\}$.
	}
	\label{alg:semibiased}
	\begin{algorithmic}[1]
	  \For{$k \gets 1$ to $M$}
	    \For{$t \gets 1$ to $S'$}
	      \State $\bz_{i_k}^t \sim q_{\phi_{i_k}}(\bz_{i_k})$
	      \State $u \sim {\rm Uniform}(0,1)$
		  \State $\mathrm{acc}_k^t  \gets u < a_{\bphi_{i_k}, \bth}(\bz_{i_k})$
	    \EndFor
	    \State $\mathrm{j}_{1:S'} \gets \mathrm{argsort}(\mathrm{acc}_k^{1:S'})$
	    \For{$t \gets 1$ to $S'$}
	      \State $\bz_{i_k}^t \gets \bz_{i_k}^{j_{S-t + 1}}$
	      \State $\mathrm{acc}_{k}^t \gets \mathrm{acc}_{k}^{j_{S-t + 1}}$
	    \EndFor
	  \EndFor
	  \State return $\{\bz_{i_1}^{1:S},\ldots,\bz_{i_M}^{1:S}\}$, $\{\mathrm{acc}_1^{1:S},\ldots,\mathrm{acc}_M^{1:S}\}$
	\end{algorithmic}
\end{algorithm}

